Controlling the rheo-electric properties of graphite/carbon black suspensions by 'flow-switching'

The ability to manipulate rheological and electrical properties of colloidal carbon black gels makes them attractive in composites for energy applications such as batteries and fuel cells, where they conduct electricity and prevent sedimentation of `granular' active components. While it is commonly assumed that granular fillers have a simple additive effect on the composite properties, new phenomena can emerge unexpectedly, with some composites exhibiting a unique rheological bi-stability between solid-like and liquid-like states. Here we report such bi-stability in suspensions of non-Brownian graphite and colloidal carbon black in oil, a model system to mimic composite suspensions for energy applications. Steady shear below a critical stress elicits a transition to a persistent mechanically weak and poorly conducting state, which must be `rejuvenated' using high-stress shear to recover a stronger, high-conductivity state. Our findings highlight the highly tunable nature of binary granular/gel composite suspensions, and present new possibilities for optimizing mixing and processing conditions for Li-ion battery slurries.

==> Sections/Methods.tex <==
\section*{Methods}

\textbf{Suspension preparation.} The synthetic graphite (Timrex KS150) and carbon black (Ensaco 250G) were kindly provided by Imerys Graphite \& Carbon (Bodio, Switzerland). Using vibrational sieving, the fraction of graphite powder passing through a $63 \ \si{\mu m}$ aperture was collected and used for the investigations. The heavy mineral oil (Merck 330760; viscosity $\eta_0 = \SI{0.14}{\pascal\second}$ at \SI{25}{\celsius}) was obtained from Merck.\\
Carbon black powder was mixed with the mineral oil in a blue cap bottle by shaking the mixture and subsequently placing the bottle in a sonication bath (Bransonic 5510E-MT, frequency \SI{42}{kHz} and \SI{135}{W}) for one hour. To prepare the binary suspensions, the gel was manually mixed with the graphite powder, and the resulting binary suspension was vigorously mixed before being loaded into the rheometer. The samples were stored at room temperature and shaken and stirred vigorously before performing the measurements.

\textbf{Rheometry.} Rheological measurements were conducted with a stress-controlled AR-G2 rheometer (TA Instruments) with the temperature kept at \SI{23}{\celsius} using a Peltier plate. A crosshatched parallel plate geometry (diameter \SI{40}{\milli\meter}, gap height \SI{800}{\micro\meter}) was used for the measurements. To erase memory of the loading history, the CB gel and binary suspensions were sheared at $\dot{\gamma} = 1000 \ \si{s^{-1}}$ for up to \SI{1200}{s} to allow the viscosity to reach a plateau unless otherwise stated. We visually checked for sample fracture which remained absent in our samples.

\textbf{Cryo-SEM.} The scanning electron microscope (SEM) was a Zeiss Crossbeam 550 FIB-SEM with a Quorum Technologies Ltd PP3010T cryogenic attachment. After shearing the samples on the rheometer, the upper geometry was lifted and a small amount of sample was carefully transferred and spaced between two rivets. The rivets were placed in the sample holder and plunge frozen into slush nitrogen before being loaded into the Quorum chamber. We freeze fractured the samples inside the Quorum chamber at \SI{-140}{\celsius}. Afterwards, a \SI{5}{min} sublimation at \SI{-90}{\celsius} was performed. The sample was not coated for imaging, and the acceleration voltage was \SI{1}{kV}. The Zeiss 'InLens' secondary electron detector, located in the electron column, along with the secondary electron secondary ion (SESI) detector was used to acquire the micrographs.\\
Monte Carlo simulations were performed with the software CASINO (v3.3.0.4) to estimate secondary electron yields from the constituents of our sample. A density of \SI{2.22}{g \ cm^3} was used for the graphite (as measured by the manufacturer), and paraffins consisting of 14, 29 and 43 carbon atoms were used to model the mineral oil with density \SI{0.87}{g \ cm^3}. Similar to the experiments, the acceleration voltage was \SI{1}{kV} and beam diameter \SI{1.5}{nm} in the simulations.

\textbf{Dielectric characterization.} An HR-20 rheometer (TA Instruments) fitted with a dielectric accessory was used for electrical and rheoeletrical measurements. A smooth parallel plate geometry (diameter \SI{25}{\milli\meter}, gap height \SI{800}{\micro\meter}) and an LCR meter (Keysight E4980A) with a frequency range of \SI{20}{Hz} to \SI{2}{MHz} were used for the dielectric measurements. Short-circuit and open measurements were conducted to correct the measured data. For the analysis, we only consider the real part of the complex conductivity, $\mathrm{Re} \left(\sigma^*\right) = \sigma' = \omega \epsilon_r'' \epsilon_0$, where $\epsilon_r''$ is the imaginary part of the complex permittivity and $\epsilon_0 \simeq 8.854\cdot 10^{-12} \ \si{F \cdot m^{-1}}$ the permittivity of free space, obtained at an AC voltage of \SI{100}{mV}. Both $\sigma'\left(\omega \right)$ and $\epsilon_{\rm r}''\left(\omega \right)$ are shown in Figure S1 in the supplementary information (SI). To obtain the direct current (dc) conductivity, $\sigma_{\rm dc}$, we fit the conductivity spectra by $\epsilon_{\rm r}'' = \sigma_{\rm dc}/ \left(\omega  \epsilon_0\right)$ in the frequency range 20-1000 Hz and 20-250 Hz for the composite and gel, respectively, since $\epsilon_{\rm r}''\left(\omega \right)$ exhibits a slope of -1 \cite{book:Schonhals2003}. A minimum of two spectra were collected for each sample.

